Graph Enhanced BERT for Query Understanding

Query understanding plays a key role in exploring users' search intents and facilitating users to locate their most desired information. However, it is inherently challenging since it needs to capture semantic information from short and ambiguous queries and often requires massive task-specific labeled data. In recent years, pre-trained language models (PLMs) have advanced various natural language processing tasks because they can extract general semantic information from large-scale corpora. Therefore, there are unprecedented opportunities to adopt PLMs for query understanding. However, there is a gap between the goal of query understanding and existing pre-training strategies -- the goal of query understanding is to boost search performance while existing strategies rarely consider this goal. Thus, directly applying them to query understanding is sub-optimal. On the other hand, search logs contain user clicks between queries and urls that provide rich users' search behavioral information on queries beyond their content. Therefore, in this paper, we aim to fill this gap by exploring search logs. In particular, to incorporate search logs into pre-training, we first construct a query graph where nodes are queries and two queries are connected if they lead to clicks on the same urls. Then we propose a novel graph-enhanced pre-training framework, GE-BERT, which can leverage both query content and the query graph. In other words, GE-BERT can capture both the semantic information and the users' search behavioral information of queries. Extensive experiments on various query understanding tasks have demonstrated the effectiveness of the proposed framework.

==> 2_relatework.tex <==
\section{Related Work}
\label{sec:related_work}
In this section, we briefly reviews related work, including the query understanding tasks, general pre-training models, and various graph neural networks.
\subsection{Query Understanding}

To explore users' query intents, researchers have conducted extensive studies from different perspectives, such as query classification~\cite{shen2006query, zhou2017survey}, query matching~\cite{li2014semantic}, query suggestion~\cite{wu2018query,anagnostopoulos2010optimization,mei2008query}, query expansion~\cite{zheng2020bert}, etc. Among them, query classification is an efective way to understand queries, which can straightforwardly improve the quality of Web search results. 
% Early works of query classification are mainly intent-based or topic-based~\cite{brenes2009survey}. Query intent classification potentially aims at identifying the underlying goal of the submitted query~\cite{broder2002taxonomy,rose2004understanding}. %Broder et al.~\cite{broder2002taxonomy} first defined three types of query intents: navigational, informational, and transactional. Rose et al.~\cite{rose2004understanding} further proposed a more complex classification of query types by introducing subcategories of informational queries and transactional queries. 
% On the other hand, 
Query  classification tries to categorize a query into a predefined taxonomy based on the topic~\cite{beitzel2005improving, cao2009context, broder2007robust,yang2015learning,shi2016deep}.
%Previous studies considered local information, query context and external Web knowledge to classify queries heuristically~\cite{beitzel2005improving, cao2009context, broder2007robust}. Recent works~\cite{yang2015learning,shi2016deep} explored to learn embedding vectors based on various types of  neural networks. 
Furthermore, query matching is another practical task for search engines, which aims to predict if two given queries have similar semantic meaning. 

\subsection{Pre-training Techniques}
Strategies for learning pre-training language representations can be divided into two categories: feature-based and fine-tuning.  Feature-based methods~\cite{mikolov2013distributed,pennington2014glove,peters2018deep} generally adopt  features to learn word embeddings. 
For example, ELMo~\cite{peters2018deep} takes the pre-training representatios as additional features and generates high-quality deep context-aware emebddings, in which the word polysemy issue has been addressed.
For fine-tuning based methods~\cite{radford2018improving, DevlinCLT19}, the goal is to provide a good pre-trained architecture that is used as a starting point for specific downstream tasks. The pre-trained model captures rich semantic patterns by training on large-scale corpus. %It acts as a regularizer and gives consistently better generalization from the training dataset~\cite{erhan2010does}. 
Recent works~\cite{yu2020technical,ramachandran2016unsupervised} have shown their effectiveness in various natural language processing areas.
A notable example is BERT~\cite{DevlinCLT19}, which is built on the transformer architecture~\cite{vaswani2017attention}.
%and leverages the masked language model to learn bidirectional representations. 
Recently, the effectiveness of BERT has also been explored in query understanding tasks~\cite{zheng2020bert,mustar2020using, chen2019bert,liu2020deep}. 
For example, Zheng et al.~\cite{zheng2020bert} proposed a query expansion model that leverages BERT to select relevant document chunks for expansion.
% Liu et al.~\cite{liu2020deep} proposed to use the pre-trained BERT model with the LinkedIn data for query classification.
Mustar et al.~\cite{mustar2020using} showed that BERT exhibits more robust to noise and has a better understanding of complex queries than conventional methods for the query suggestion task. 




\subsection{Graph Neural Networks}
Classical GNNs~\cite{BrunaZSL13, DefferrardBV16, KipfW17} are typically based on spectral methods, which generally define the convolutional operations in the Fourier domain. An efficient and simplified example is GCN~\cite{KipfW17}, which extends the convolution operator by approximating the first-order Chebyshev expansion.
Modern GNNs~\cite{HamiltonYL17, VelickovicCCRLB18}  are built upon neural networks that learn representation vectors on the graph-structured data. They generally pass information from a target node to the next layer via propagation and aggregation on its neighbors. 
Among them, 
% Hamilton et al. ~\cite{HamiltonYL17} proposed the GraphSAGE model, which conducts aggregations on a fixed size of neighbors.
Velickovic et al.~\cite{VelickovicCCRLB18} proposed the GAT model that applies the attention mechanism to aggregate representations on the entire neighborhood.
% Nowadays, GNNs have been extended to work on various types of graphs, including social networks~\cite{Fan0LHZTY19}, knowledge graphs~\cite{wang2018cross}, biological molecules~\cite{DuvenaudMABHAA15}, point cloud~\cite{hassani2019unsupervised}, etc.
Inspired by the great success of GNNs, we adopt GNN to integrate  the query graph information for accurately modeling.

